MultiVerS: Improving scientific claim verification with weak supervision and full-document context

The scientific claim verification task requires an NLP system to label scientific documents which Support or Refute an input claim, and to select evidentiary sentences (or rationales) justifying each predicted label. In this work, we present MultiVerS, which predicts a fact-checking label and identifies rationales in a multitask fashion based on a shared encoding of the claim and full document context. This approach accomplishes two key modeling goals. First, it ensures that all relevant contextual information is incorporated into each labeling decision. Second, it enables the model to learn from instances annotated with a document-level fact-checking label, but lacking sentence-level rationales. This allows MultiVerS to perform weakly-supervised domain adaptation by training on scientific documents labeled using high-precision heuristics. Our approach outperforms two competitive baselines on three scientific claim verification datasets, with particularly strong performance in zero / few-shot domain adaptation experiments. Our code and data are available at https://github.com/dwadden/multivers.

==> _old_sec-introduction.tex <==
\section{Introduction} \label{sec:intro}

\input{fig/teaser-wrapper.tex}

The task of scientific claim verification requires a system to assess the veracity of a scientific claim against a corpus of documents. The proliferation of mis- and dis-information on the web -- particularly as it relates the COVID-19 pandemic \cite{Pennycook2020FightingCM, Naeem2020AnEO} -- has motivated the release of a number of new datasets for this task \cite{Saakyan2021COVIDFactFE,Sarrouti2021EvidencebasedFO,Wadden2020FactOF,Kotonya2020ExplainableAF}, accompanied by advances in model performance \cite{Pradeep2021ScientificCV,Li2021APM,Zhang2021AbstractRS}.

Given a claim and an abstract that may contain evidence, existing scientific claim verification systems first extract rationales from the abstract which contain evidence sufficient to entail or contradict the claim, when taken in the context of the abstract. Then, they predict a fact-checking label based on a representation of the selected rationales. This ``extract-then-label'' approach has two potential drawbacks. First, the rationales containing evidence may lack information required to make a prediction out-of-context; for instance, they may contain acronyms or pronouns, or lack qualifiers that specify the scope of a reported finding. Figure \ref{fig:teaser} provides an example. This challenge has previously been observed in work on scientific literature understanding \cite{Nye2020UnderstandingCT}, and has been studied more generally in the task of sentence \emph{decontextualization} \cite{Choi2021DecontextualizationMS}. We describe existing approaches to mitigate this issue in \S \ref{sec:model_bg}.

Second, the ``extract-then-label'' approach requires training data annotated with both sentence-level rationales and abstract-level labels. While sentence-level annotations for scientific claim verification are costly, abstract-level labels can be created cheaply using high-precision heuristics. For instance, the titles of research papers often make claims that are supported by their abstracts. Ideally, models should be able to take advantage of these additional abstract-level labels without requiring that they be paired with rationale annotations.

Motivated by these challenges, we develop \sysname: given a claim and evidence-containing abstract, \sysname encodes the entire claim / abstract context in a single long sequence. The resulting context exceeds the 512-token window common to \bert-style \cite{Devlin2019BERTPO} transformer architectures between 12\% and 43\% of the time, depending on dataset. To accommodate this, \sysname builds on the \longformer model, which has been successfully applied to related tasks, such as question answering, involving long-document context \cite{Beltagy2020LongformerTL,Pradeep2021ScientificCV}. 

\longformer uses specialized sentinel tokens to construct globally-contextualized representations of the entire context, and each individual sentence in the abstract. We use these representations to predict an abstract-level fact-checking label and sentence-level rationales in a multitask fashion, enforcing consistency between the outputs of the two tasks during decoding. We find that this modeling approach improves performance on three datasets for scientific claim verification over two state-of-the-art baselines, one of which has more than 10x the parameters of our system. In addition, it is able to effectively leverage weakly-labeled in-domain data for zero / few-shot domain adaptation.

In summary, we make the following contributions: (1) We introduce \sysname, a multitask system for full-context scientific claim verification, and find that it outperforms two state-of-the-art baselines on three datasets. (2) We propose simple heuristics to assign fact-checking labels to two large scientific datasets, and show that training on these annotations enables zero and few-shot domain adaptation. (3) We conduct ablations and analysis to characterize the performance contributions of our modeling approach and training procedure.


==> sec-introduction-unified.tex <==
The proliferation of scientific mis- and dis-information on the web -- particularly as it relates to the COVID-19 pandemic -- has motivated the release of a number of new datasets \cite{Saakyan2021COVIDFactFE,Sarrouti2021EvidencebasedFO,Wadden2020FactOF,Kotonya2020ExplainableAF} and the development of modeling approaches \cite{Pradeep2021ScientificCV,Li2021APM,Zhang2021AbstractRS} for the task of \emph{scientific claim verification}. 


The proliferation of scientific mis- and dis-information on the web -- particularly as it relates to the COVID-19 pandemic -- has spurred research activity on the task of \emph{scientific claim verification}. Broadly speaking, this task requires an NLP system to assess the veracity of a scientific claim against a textual context. A number of datasets have been released to facilitate progress on this task  \cite{Saakyan2021COVIDFactFE,Sarrouti2021EvidencebasedFO,Wadden2020FactOF,Kotonya2020ExplainableAF}. While these datasets all focus on scientific claim verification, they are formulated in different ways. Some datasets treat fact verification as a textual entailment task, asking systems to predict whether a claim is entailed or contradicted by a single sentence found in a scientific document. Others formulate it as a multi-step process involving retrieval of relevant documents, labeling whether the retrieved documents \support or \refute the input claim, and extracting rationales from the retrieved documents which justify the predicted label.

In addition, due to the difficulty of collecting expert fact-checking annotations in specialized domains, all existing datasets are relatively small in size, and / or rely on relatively noisy heuristics to generate important dataset features -- such as claims \refuted rather than \supported by the evidence. On the other hand, large corpora of unlabeled scientific documents could potentially be leveraged additional as supervision on this task.

In this work, we propose to unify these existing datasets into one approach and develop a model that is able to incorporate all forms of supervision from all available data, etc. etc. 








==> table/ablations_1col_architecture_raw.tex <==
\begin{tabular}{lllll}
\toprule
                 &         &                      healthver &                      covidfact &                        scifact \\
Setting & Architecture &                                &                                &                                \\
\midrule
\multirow{3}{*}{Zero-shot} & Multitask &   \textbf{30.7} / \textbf{7.8} &  \textbf{47.2} / \textbf{23.6} &  \textbf{46.7} / \textbf{27.8} \\
                 & Pipe &                      3.2 / 0.9 &                    19.0 / 10.5 &                    22.5 / 12.8 \\
                 & MT / PI &                      4.5 / 1.8 &                    26.7 / 13.5 &                    28.3 / 17.7 \\
\cline{1-5}
\multirow{3}{*}{Few-shot} & Multitask &  \textbf{54.7} / \textbf{35.7} &           \textbf{69.7} / 37.4 &  \textbf{63.3} / \textbf{45.3} \\
                 & Pipe &                    52.8 / 29.5 &           68.3 / \textbf{38.2} &                    53.0 / 39.9 \\
                 & MT / PI &                    46.7 / 32.3 &                    59.3 / 34.1 &                    56.2 / 41.1 \\
\cline{1-5}
\multirow{3}{*}{Fully-supervised} & Multitask &                    77.6 / 69.1 &                    77.3 / 43.7 &  \textbf{72.5} / \textbf{67.2} \\
                 & Pipe &  \textbf{78.4} / \textbf{69.2} &  \textbf{77.6} / \textbf{47.7} &                    70.9 / 66.2 \\
                 & MT / PI &                    70.6 / 64.3 &                    73.3 / 44.0 &                    60.3 / 57.0 \\
\bottomrule
\end{tabular}


==> table/ablations_1col_encoder_raw.tex <==
\begin{tabular}{lllll}
\toprule
                 &         &                      healthver &                      covidfact &                        scifact \\
Setting & Encoder &                                &                                &                                \\
\midrule
\multirow{2}{*}{Zero-shot} & Longformer &                     30.7 / 7.8 &                    47.2 / 23.6 &  \textbf{46.7} / \textbf{27.8} \\
                 & RoBERTa &   \textbf{34.2} / \textbf{9.2} &  \textbf{48.3} / \textbf{26.2} &                    45.2 / 25.9 \\
\cline{1-5}
\multirow{2}{*}{Few-shot} & Longformer &           \textbf{54.7} / 35.7 &                    69.7 / 37.4 &  \textbf{63.3} / \textbf{45.3} \\
                 & RoBERTa &           51.2 / \textbf{36.9} &  \textbf{72.1} / \textbf{41.0} &                    50.5 / 34.0 \\
\cline{1-5}
\multirow{2}{*}{Fully-supervised} & Longformer &                    77.6 / 69.1 &           77.3 / \textbf{43.7} &  \textbf{72.5} / \textbf{67.2} \\
                 & RoBERTa &  \textbf{78.8} / \textbf{72.7} &           \textbf{78.2} / 43.4 &                    67.6 / 62.3 \\
\bottomrule
\end{tabular}


==> table/ablations_1col_pretraining_raw.tex <==
\begin{tabular}{lllll}
\toprule
                 &      &                      healthver &                      covidfact &                        scifact \\
Setting & Pretraining &                                &                                &                                \\
\midrule
\multirow{2}{*}{Zero-shot} & All &   \textbf{30.7} / \textbf{7.8} &  \textbf{47.2} / \textbf{23.6} &  \textbf{46.7} / \textbf{27.8} \\
                 & Fever &                      1.3 / 0.7 &                    25.2 / 11.2 &                    23.9 / 11.8 \\
\cline{1-5}
\multirow{3}{*}{Few-shot} & All &  \textbf{54.7} / \textbf{35.7} &                    69.7 / 37.4 &  \textbf{63.3} / \textbf{45.3} \\
                 & Fever &                    53.4 / 31.9 &  \textbf{74.4} / \textbf{42.1} &                    54.5 / 39.0 \\
                 & None &                    39.4 / 27.0 &                    67.8 / 22.6 &                    24.2 / 10.8 \\
\cline{1-5}
\multirow{3}{*}{Fully-supervised} & All &           \textbf{77.6} / 69.1 &           77.3 / \textbf{43.7} &  \textbf{72.5} / \textbf{67.2} \\
                 & Fever &           77.1 / \textbf{70.3} &           \textbf{77.4} / 43.3 &                    67.9 / 61.7 \\
                 & None &                    74.5 / 69.7 &                    69.7 / 36.6 &                    63.3 / 58.4 \\
\bottomrule
\end{tabular}


==> table/ablations_full_architecture_raw.tex <==
\begin{tabular}{llllllllllllllllllllll}
\toprule
                 & {} & abstract_label_only_precision & abstract_label_only_recall & abstract_label_only_f1 & sentence_label_precision & sentence_label_recall & sentence_label_f1 & blank_8 & abstract_label_only_precision & abstract_label_only_recall & abstract_label_only_f1 & sentence_label_precision & sentence_label_recall & sentence_label_f1 & blank_14 & abstract_label_only_precision & abstract_label_only_recall & abstract_label_only_f1 & sentence_label_precision & sentence_label_recall & sentence_label_f1 \\
                 & dataset &                     healthver &                  healthver &              healthver &                healthver &             healthver & \multicolumn{2}{l}{healthver} &                     covidfact &                  covidfact &              covidfact &                covidfact &             covidfact & \multicolumn{2}{l}{covidfact} &                       scifact &                    scifact &                scifact &                  scifact &               scifact &           scifact \\
Setting & Architecture &                               &                            &                        &                          &                       &                   &         &                               &                            &                        &                          &                       &                   &          &                               &                            &                        &                          &                       &                   \\
\midrule
\multirow{3}{*}{Zero-shot} & Multitask &                     \sz{60.6} &                  \sz{20.5} &          \textbf{30.7} &                \sz{25.0} &              \sz{4.6} &      \textbf{7.8} &         &                     \sz{48.8} &                  \sz{45.7} &          \textbf{47.2} &                \sz{32.7} &             \sz{18.5} &     \textbf{23.6} &          &                     \sz{49.0} &                  \sz{44.6} &          \textbf{46.7} &                \sz{39.0} &             \sz{21.6} &     \textbf{27.8} \\
                 & Pipe &                     \sz{58.8} &                   \sz{1.7} &                    3.2 &                \sz{29.4} &              \sz{0.5} &               0.9 &         &                     \sz{67.3} &                  \sz{11.0} &                     19 &                \sz{57.4} &              \sz{5.8} &              10.5 &          &                     \sz{80.6} &                  \sz{13.1} &                   22.5 &                \sz{72.2} &              \sz{7.0} &              12.8 \\
                 & MT / PI &                     \sz{60.9} &                   \sz{2.3} &                    4.5 &                \sz{41.7} &              \sz{0.9} &               1.8 &         &                     \sz{78.5} &                  \sz{16.1} &                   26.7 &                \sz{57.7} &              \sz{7.6} &              13.5 &          &                     \sz{80.9} &                  \sz{17.1} &                   28.3 &                \sz{75.5} &             \sz{10.0} &              17.7 \\
\cline{1-22}
\multirow{3}{*}{Few-shot} & Multitask &                     \sz{63.6} &                  \sz{47.9} &          \textbf{54.7} &                \sz{41.9} &             \sz{31.0} &     \textbf{35.7} &         &                     \sz{71.3} &                  \sz{68.1} &          \textbf{69.7} &                \sz{39.5} &             \sz{35.4} &              37.4 &          &                     \sz{76.4} &                  \sz{54.1} &          \textbf{63.3} &                \sz{51.7} &             \sz{40.3} &     \textbf{45.3} \\
                 & Pipe &                     \sz{56.3} &                  \sz{49.7} &                   52.8 &                \sz{32.6} &             \sz{27.0} &              29.5 &         &                     \sz{69.4} &                  \sz{67.2} &                   68.3 &                \sz{40.6} &             \sz{36.0} &     \textbf{38.2} &          &                     \sz{54.8} &                  \sz{51.4} &                     53 &                \sz{43.7} &             \sz{36.8} &              39.9 \\
                 & MT / PI &                     \sz{67.0} &                  \sz{35.9} &                   46.7 &                \sz{44.5} &             \sz{25.3} &              32.3 &         &                     \sz{72.6} &                  \sz{50.2} &                   59.3 &                \sz{40.2} &             \sz{29.7} &              34.1 &          &                     \sz{85.3} &                  \sz{41.9} &                   56.2 &                \sz{54.7} &             \sz{33.0} &              41.1 \\
\cline{1-22}
\multirow{3}{*}{Fully-supervised} & Multitask &                     \sz{78.9} &                  \sz{76.3} &                   77.6 &                \sz{71.4} &             \sz{67.0} &              69.1 &         &                     \sz{77.3} &                  \sz{77.3} &                   77.3 &                \sz{41.5} &             \sz{46.1} &              43.7 &          &                     \sz{73.8} &                  \sz{71.2} &          \textbf{72.5} &                \sz{67.4} &             \sz{67.0} &     \textbf{67.2} \\
                 & Pipe &                     \sz{78.7} &                  \sz{78.1} &          \textbf{78.4} &                \sz{70.2} &             \sz{68.3} &     \textbf{69.2} &         &                     \sz{79.9} &                  \sz{75.4} &          \textbf{77.6} &                \sz{48.2} &             \sz{47.2} &     \textbf{47.7} &          &                     \sz{68.5} &                  \sz{73.4} &                   70.9 &                \sz{64.5} &             \sz{68.1} &              66.2 \\
                 & MT / PI &                     \sz{77.6} &                  \sz{64.8} &                   70.6 &                \sz{70.0} &             \sz{59.5} &              64.3 &         &                     \sz{77.7} &                  \sz{69.4} &                   73.3 &                \sz{43.6} &             \sz{44.4} &                44 &          &                     \sz{80.5} &                  \sz{48.2} &                   60.3 &                \sz{70.5} &             \sz{47.8} &                57 \\
\bottomrule
\end{tabular}


==> table/ablations_full_encoder_raw.tex <==
\begin{tabular}{llllllllllllllllllllll}
\toprule
                 & {} & abstract_label_only_precision & abstract_label_only_recall & abstract_label_only_f1 & sentence_label_precision & sentence_label_recall & sentence_label_f1 & blank_8 & abstract_label_only_precision & abstract_label_only_recall & abstract_label_only_f1 & sentence_label_precision & sentence_label_recall & sentence_label_f1 & blank_14 & abstract_label_only_precision & abstract_label_only_recall & abstract_label_only_f1 & sentence_label_precision & sentence_label_recall & sentence_label_f1 \\
                 & dataset &                     healthver &                  healthver &              healthver &                healthver &             healthver & \multicolumn{2}{l}{healthver} &                     covidfact &                  covidfact &              covidfact &                covidfact &             covidfact & \multicolumn{2}{l}{covidfact} &                       scifact &                    scifact &                scifact &                  scifact &               scifact &           scifact \\
Setting & Encoder &                               &                            &                        &                          &                       &                   &         &                               &                            &                        &                          &                       &                   &          &                               &                            &                        &                          &                       &                   \\
\midrule
\multirow{2}{*}{Zero-shot} & Longformer &                     \sz{60.6} &                  \sz{20.5} &                   30.7 &                \sz{25.0} &              \sz{4.6} &               7.8 &         &                     \sz{48.8} &                  \sz{45.7} &                   47.2 &                \sz{32.7} &             \sz{18.5} &              23.6 &          &                     \sz{49.0} &                  \sz{44.6} &          \textbf{46.7} &                \sz{39.0} &             \sz{21.6} &     \textbf{27.8} \\
                 & RoBERTa &                     \sz{59.5} &                  \sz{24.0} &          \textbf{34.2} &                \sz{25.4} &              \sz{5.6} &      \textbf{9.2} &         &                     \sz{49.3} &                  \sz{47.3} &          \textbf{48.3} &                \sz{35.2} &             \sz{20.9} &     \textbf{26.2} &          &                     \sz{45.5} &                  \sz{45.0} &                   45.2 &                \sz{34.4} &             \sz{20.8} &              25.9 \\
\cline{1-22}
\multirow{2}{*}{Few-shot} & Longformer &                     \sz{63.6} &                  \sz{47.9} &          \textbf{54.7} &                \sz{41.9} &             \sz{31.0} &              35.7 &         &                     \sz{71.3} &                  \sz{68.1} &                   69.7 &                \sz{39.5} &             \sz{35.4} &              37.4 &          &                     \sz{76.4} &                  \sz{54.1} &          \textbf{63.3} &                \sz{51.7} &             \sz{40.3} &     \textbf{45.3} \\
                 & RoBERTa &                     \sz{55.0} &                  \sz{47.9} &                   51.2 &                \sz{39.0} &             \sz{35.0} &     \textbf{36.9} &         &                     \sz{72.5} &                  \sz{71.6} &          \textbf{72.1} &                \sz{39.7} &             \sz{42.5} &     \textbf{41.0} &          &                     \sz{59.0} &                  \sz{44.1} &                   50.5 &                \sz{36.8} &             \sz{31.6} &                34 \\
\cline{1-22}
\multirow{2}{*}{Fully-supervised} & Longformer &                     \sz{78.9} &                  \sz{76.3} &                   77.6 &                \sz{71.4} &             \sz{67.0} &              69.1 &         &                     \sz{77.3} &                  \sz{77.3} &                   77.3 &                \sz{41.5} &             \sz{46.1} &     \textbf{43.7} &          &                     \sz{73.8} &                  \sz{71.2} &          \textbf{72.5} &                \sz{67.4} &             \sz{67.0} &     \textbf{67.2} \\
                 & RoBERTa &                     \sz{77.8} &                  \sz{80.0} &          \textbf{78.8} &                \sz{73.4} &             \sz{72.0} &     \textbf{72.7} &         &                     \sz{78.2} &                  \sz{78.2} &          \textbf{78.2} &                \sz{40.8} &             \sz{46.3} &              43.4 &          &                     \sz{67.1} &                  \sz{68.0} &                   67.6 &                \sz{62.7} &             \sz{61.9} &              62.3 \\
\bottomrule
\end{tabular}


==> table/ablations_full_pretraining_raw.tex <==
\begin{tabular}{llllllllllllllllllllll}
\toprule
                 & {} & abstract_label_only_precision & abstract_label_only_recall & abstract_label_only_f1 & sentence_label_precision & sentence_label_recall & sentence_label_f1 & blank_8 & abstract_label_only_precision & abstract_label_only_recall & abstract_label_only_f1 & sentence_label_precision & sentence_label_recall & sentence_label_f1 & blank_14 & abstract_label_only_precision & abstract_label_only_recall & abstract_label_only_f1 & sentence_label_precision & sentence_label_recall & sentence_label_f1 \\
                 & dataset &                     healthver &                  healthver &              healthver &                healthver &             healthver & \multicolumn{2}{l}{healthver} &                     covidfact &                  covidfact &              covidfact &                covidfact &             covidfact & \multicolumn{2}{l}{covidfact} &                       scifact &                    scifact &                scifact &                  scifact &               scifact &           scifact \\
Setting & Pretraining &                               &                            &                        &                          &                       &                   &         &                               &                            &                        &                          &                       &                   &          &                               &                            &                        &                          &                       &                   \\
\midrule
\multirow{2}{*}{Zero-shot} & All &                     \sz{60.6} &                  \sz{20.5} &          \textbf{30.7} &                \sz{25.0} &              \sz{4.6} &      \textbf{7.8} &         &                     \sz{48.8} &                  \sz{45.7} &          \textbf{47.2} &                \sz{32.7} &             \sz{18.5} &     \textbf{23.6} &          &                     \sz{49.0} &                  \sz{44.6} &          \textbf{46.7} &                \sz{39.0} &             \sz{21.6} &     \textbf{27.8} \\
                 & Fever &                     \sz{80.0} &                   \sz{0.7} &                    1.3 &                \sz{66.7} &              \sz{0.4} &               0.7 &         &                     \sz{95.8} &                  \sz{14.5} &                   25.2 &                \sz{63.5} &              \sz{6.2} &              11.2 &          &                     \sz{83.8} &                  \sz{14.0} &                   23.9 &                \sz{64.9} &              \sz{6.5} &              11.8 \\
\cline{1-22}
\multirow{3}{*}{Few-shot} & All &                     \sz{63.6} &                  \sz{47.9} &          \textbf{54.7} &                \sz{41.9} &             \sz{31.0} &     \textbf{35.7} &         &                     \sz{71.3} &                  \sz{68.1} &                   69.7 &                \sz{39.5} &             \sz{35.4} &              37.4 &          &                     \sz{76.4} &                  \sz{54.1} &          \textbf{63.3} &                \sz{51.7} &             \sz{40.3} &     \textbf{45.3} \\
                 & Fever &                     \sz{56.4} &                  \sz{50.8} &                   53.4 &                \sz{34.8} &             \sz{29.4} &              31.9 &         &                     \sz{74.4} &                  \sz{74.4} &          \textbf{74.4} &                \sz{39.3} &             \sz{45.3} &     \textbf{42.1} &          &                     \sz{72.4} &                  \sz{43.7} &                   54.5 &                \sz{48.8} &             \sz{32.4} &                39 \\
                 & None &                     \sz{38.5} &                  \sz{40.4} &                   39.4 &                \sz{28.5} &             \sz{25.7} &                27 &         &                     \sz{67.8} &                  \sz{67.8} &                   67.8 &                \sz{24.9} &             \sz{20.7} &              22.6 &          &                     \sz{20.0} &                  \sz{30.6} &                   24.2 &                 \sz{9.5} &             \sz{12.7} &              10.8 \\
\cline{1-22}
\multirow{3}{*}{Fully-supervised} & All &                     \sz{78.9} &                  \sz{76.3} &          \textbf{77.6} &                \sz{71.4} &             \sz{67.0} &              69.1 &         &                     \sz{77.3} &                  \sz{77.3} &                   77.3 &                \sz{41.5} &             \sz{46.1} &     \textbf{43.7} &          &                     \sz{73.8} &                  \sz{71.2} &          \textbf{72.5} &                \sz{67.4} &             \sz{67.0} &     \textbf{67.2} \\
                 & Fever &                     \sz{77.5} &                  \sz{76.6} &                   77.1 &                \sz{70.8} &             \sz{69.8} &     \textbf{70.3} &         &                     \sz{77.5} &                  \sz{77.3} &          \textbf{77.4} &                \sz{40.6} &             \sz{46.5} &              43.3 &          &                     \sz{64.3} &                  \sz{72.1} &                   67.9 &                \sz{57.1} &             \sz{67.0} &              61.7 \\
                 & None &                     \sz{75.0} &                  \sz{74.0} &                   74.5 &                \sz{71.8} &             \sz{67.8} &              69.7 &         &                     \sz{69.7} &                  \sz{69.7} &                   69.7 &                \sz{35.3} &             \sz{38.1} &              36.6 &          &                     \sz{64.9} &                  \sz{61.7} &                   63.3 &                \sz{62.7} &             \sz{54.6} &              58.4 \\
\bottomrule
\end{tabular}


==> table/ablations_full_raw.tex <==
\begin{tabular}{llllllrllrllrllrllrllr}
\toprule
          Setting & Architecture &     Encoder & Pretraining & abstract_label_only_precision & abstract_label_only_recall & abstract_label_only_f1 & sentence_label_precision & sentence_label_recall & sentence_label_f1 & abstract_label_only_precision & abstract_label_only_recall & abstract_label_only_f1 & sentence_label_precision & sentence_label_recall & sentence_label_f1 & abstract_label_only_precision & abstract_label_only_recall & abstract_label_only_f1 & sentence_label_precision & sentence_label_recall & sentence_label_f1 \\
                  &                     healthver &                  healthver &              healthver &                healthver &             healthver &         healthver &                     covidfact &                  covidfact &              covidfact &                covidfact &             covidfact &         covidfact &                       scifact &                    scifact &                scifact &                  scifact &               scifact &           scifact \\
        Zero-shot &    Multitask &  Longformer &         All &                     \sz{60.6} &                  \sz{20.5} &                   30.7 &                \sz{25.0} &              \sz{4.6} &               7.8 &                     \sz{48.8} &                  \sz{45.7} &                   47.2 &                \sz{32.7} &             \sz{18.5} &              23.6 &                     \sz{49.0} &                  \sz{44.6} &                   46.7 &                \sz{39.0} &             \sz{21.6} &              27.8 \\
\midrule
        Zero-shot &    Multitask &  Longformer &       Fever &                     \sz{80.0} &                   \sz{0.7} &                    1.3 &                \sz{66.7} &              \sz{0.4} &               0.7 &                     \sz{95.8} &                  \sz{14.5} &                   25.2 &                \sz{63.5} &              \sz{6.2} &              11.2 &                     \sz{83.8} &                  \sz{14.0} &                   23.9 &                \sz{64.9} &              \sz{6.5} &              11.8 \\
        Zero-shot &    Multitask &     RoBERTa &         All &                     \sz{59.5} &                  \sz{24.0} &                   34.2 &                \sz{25.4} &              \sz{5.6} &               9.2 &                     \sz{49.3} &                  \sz{47.3} &                   48.3 &                \sz{35.2} &             \sz{20.9} &              26.2 &                     \sz{45.5} &                  \sz{45.0} &                   45.2 &                \sz{34.4} &             \sz{20.8} &              25.9 \\
        Zero-shot &         Pipe &  Longformer &         All &                     \sz{58.8} &                   \sz{1.7} &                    3.2 &                \sz{29.4} &              \sz{0.5} &               0.9 &                     \sz{67.3} &                  \sz{11.0} &                   19.0 &                \sz{57.4} &              \sz{5.8} &              10.5 &                     \sz{80.6} &                  \sz{13.1} &                   22.5 &                \sz{72.2} &              \sz{7.0} &              12.8 \\
        Zero-shot &      MT / PI &  Longformer &         All &                     \sz{60.9} &                   \sz{2.3} &                    4.5 &                \sz{41.7} &              \sz{0.9} &               1.8 &                     \sz{78.5} &                  \sz{16.1} &                   26.7 &                \sz{57.7} &              \sz{7.6} &              13.5 &                     \sz{80.9} &                  \sz{17.1} &                   28.3 &                \sz{75.5} &             \sz{10.0} &              17.7 \\
         Few-shot &    Multitask &  Longformer &         All &                     \sz{63.6} &                  \sz{47.9} &                   54.7 &                \sz{41.9} &             \sz{31.0} &              35.7 &                     \sz{71.3} &                  \sz{68.1} &                   69.7 &                \sz{39.5} &             \sz{35.4} &              37.4 &                     \sz{76.4} &                  \sz{54.1} &                   63.3 &                \sz{51.7} &             \sz{40.3} &              45.3 \\
         Few-shot &    Multitask &  Longformer &       Fever &                     \sz{56.4} &                  \sz{50.8} &                   53.4 &                \sz{34.8} &             \sz{29.4} &              31.9 &                     \sz{74.4} &                  \sz{74.4} &                   74.4 &                \sz{39.3} &             \sz{45.3} &              42.1 &                     \sz{72.4} &                  \sz{43.7} &                   54.5 &                \sz{48.8} &             \sz{32.4} &              39.0 \\
         Few-shot &    Multitask &  Longformer &        None &                     \sz{38.5} &                  \sz{40.4} &                   39.4 &                \sz{28.5} &             \sz{25.7} &              27.0 &                     \sz{67.8} &                  \sz{67.8} &                   67.8 &                \sz{24.9} &             \sz{20.7} &              22.6 &                     \sz{20.0} &                  \sz{30.6} &                   24.2 &                 \sz{9.5} &             \sz{12.7} &              10.8 \\
         Few-shot &    Multitask &     RoBERTa &         All &                     \sz{55.0} &                  \sz{47.9} &                   51.2 &                \sz{39.0} &             \sz{35.0} &              36.9 &                     \sz{72.5} &                  \sz{71.6} &                   72.1 &                \sz{39.7} &             \sz{42.5} &              41.0 &                     \sz{59.0} &                  \sz{44.1} &                   50.5 &                \sz{36.8} &             \sz{31.6} &              34.0 \\
         Few-shot &         Pipe &  Longformer &         All &                     \sz{56.3} &                  \sz{49.7} &                   52.8 &                \sz{32.6} &             \sz{27.0} &              29.5 &                     \sz{69.4} &                  \sz{67.2} &                   68.3 &                \sz{40.6} &             \sz{36.0} &              38.2 &                     \sz{54.8} &                  \sz{51.4} &                   53.0 &                \sz{43.7} &             \sz{36.8} &              39.9 \\
         Few-shot &      MT / PI &  Longformer &         All &                     \sz{67.0} &                  \sz{35.9} &                   46.7 &                \sz{44.5} &             \sz{25.3} &              32.3 &                     \sz{72.6} &                  \sz{50.2} &                   59.3 &                \sz{40.2} &             \sz{29.7} &              34.1 &                     \sz{85.3} &                  \sz{41.9} &                   56.2 &                \sz{54.7} &             \sz{33.0} &              41.1 \\
 Fully-supervised &    Multitask &  Longformer &         All &                     \sz{78.9} &                  \sz{76.3} &                   77.6 &                \sz{71.4} &             \sz{67.0} &              69.1 &                     \sz{77.3} &                  \sz{77.3} &                   77.3 &                \sz{41.5} &             \sz{46.1} &              43.7 &                     \sz{73.8} &                  \sz{71.2} &                   72.5 &                \sz{67.4} &             \sz{67.0} &              67.2 \\
 Fully-supervised &    Multitask &  Longformer &       Fever &                     \sz{77.5} &                  \sz{76.6} &                   77.1 &                \sz{70.8} &             \sz{69.8} &              70.3 &                     \sz{77.5} &                  \sz{77.3} &                   77.4 &                \sz{40.6} &             \sz{46.5} &              43.3 &                     \sz{64.3} &                  \sz{72.1} &                   67.9 &                \sz{57.1} &             \sz{67.0} &              61.7 \\
 Fully-supervised &    Multitask &  Longformer &        None &                     \sz{75.0} &                  \sz{74.0} &                   74.5 &                \sz{71.8} &             \sz{67.8} &              69.7 &                     \sz{69.7} &                  \sz{69.7} &                   69.7 &                \sz{35.3} &             \sz{38.1} &              36.6 &                     \sz{64.9} &                  \sz{61.7} &                   63.3 &                \sz{62.7} &             \sz{54.6} &              58.4 \\
 Fully-supervised &    Multitask &     RoBERTa &         All &                     \sz{77.8} &                  \sz{80.0} &                   78.8 &                \sz{73.4} &             \sz{72.0} &              72.7 &                     \sz{78.2} &                  \sz{78.2} &                   78.2 &                \sz{40.8} &             \sz{46.3} &              43.4 &                     \sz{67.1} &                  \sz{68.0} &                   67.6 &                \sz{62.7} &             \sz{61.9} &              62.3 \\
 Fully-supervised &         Pipe &  Longformer &         All &                     \sz{78.7} &                  \sz{78.1} &                   78.4 &                \sz{70.2} &             \sz{68.3} &              69.2 &                     \sz{79.9} &                  \sz{75.4} &                   77.6 &                \sz{48.2} &             \sz{47.2} &              47.7 &                     \sz{68.5} &                  \sz{73.4} &                   70.9 &                \sz{64.5} &             \sz{68.1} &              66.2 \\
 Fully-supervised &      MT / PI &  Longformer &         All &                     \sz{77.6} &                  \sz{64.8} &                   70.6 &                \sz{70.0} &             \sz{59.5} &              64.3 &                     \sz{77.7} &                  \sz{69.4} &                   73.3 &                \sz{43.6} &             \sz{44.4} &              44.0 &                     \sz{80.5} &                  \sz{48.2} &                   60.3 &                \sz{70.5} &             \sz{47.8} &              57.0 \\
\bottomrule
\end{tabular}


==> table/cross_train_abstract_orig.tex <==
\begin{tabular}{lrrrrrr}
\toprule
{} & \multicolumn{2}{l}{\healthVer} & \multicolumn{2}{l}{\covidFact} & \multicolumn{2}{l}{\scifact} \\
{} &         F1 &  Diff &         F1 &  Diff &       F1 &  Diff \\
\midrule
\healthVer &       86.1 &   0.0 &       50.2 & -24.0 &     73.4 & -15.8 \\
\covidFact &       50.6 & -35.6 &       74.1 &   0.0 &     76.1 & -13.1 \\
\scifact   &       70.5 & -15.7 &       54.6 & -19.6 &     89.2 &   0.0 \\
Combined   &       83.0 &  -3.2 &       64.3 &  -9.8 &     87.8 &  -1.3 \\
\bottomrule
\end{tabular}



==> table/cross_train_sent_orig.tex <==
\begin{tabular}{lrrrrrr}
\toprule
{} & \multicolumn{2}{l}{\healthVer} & \multicolumn{2}{l}{\covidFact} & \multicolumn{2}{l}{\scifact} \\
{} &         F1 &  Diff &         F1 &  Diff &       F1 &  Diff \\
\midrule
\healthVer &       74.2 &   0.0 &       28.0 & -12.6 &     39.7 & -32.4 \\
\covidFact &       14.6 & -59.5 &       40.6 &   0.0 &     41.6 & -30.6 \\
\scifact   &       20.5 & -53.7 &       33.9 &  -6.7 &     72.1 &   0.0 \\
Combined   &       71.4 &  -2.8 &       39.8 &  -0.9 &     70.5 &  -1.6 \\
\bottomrule
\end{tabular}



==> table/dataset_counts_orig.tex <==
\begin{tabular}{{p{0.12\linewidth}p{0.25\linewidth}R{0.15\linewidth}R{0.15\linewidth}R{0.15\linewidth}}}
     \toprule
                            &            & \supports & \nei & \refutes \\
     Fold                   & Dataset    &           &      &          \\
     \midrule
     \multirow{3}{*}{Train} & \scifact   & 508       & 485  & 265      \\
                            & \covidFact & 299       & -    & 641      \\
                            & \healthVer & 2384      & 2384 & 1464     \\
     \cmidrule(lr){1-5}
     \multirow{3}{*}{Eval}  & \scifact   & 113       & 127  & 109      \\
                            & \covidFact & 102       & -    & 215      \\
                            & \healthVer & 374       & 304  & 225      \\
     \bottomrule
\end{tabular}


==> table/dataset_summary_orig.tex <==
\begin{tabular}{llllrrrr}
\toprule
\tworows{Dataset} & \tworows{Domain} &    \tworows{Claim source} & \tworows{Negation \\ method} & \tworows{Train \\ claims} & \tworows{Eval \\ claims} & \tworows{> 512 \\ tokens} &  \tworows{Rationales \\ per abstract} \\
\midrule
           \fever &             Wiki &       Wikipedia sentences &                        Human &                   130,644 &                        - &                    33.2\% &                                  1.20 \\
             \pqa &           Biomed &  Automatic (Paper titles) &                    Automatic &                    58,370 &                        - &                    12.1\% &                                  0.00 \\
              \ei &           Biomed &        Automatic (prompts) &                    Automatic &                     7,395 &                        - &                    42.7\% &                                  1.10 \\
         \scifact &           Biomed &        Citation sentences &                        Human &                     1,109 &                      300 &                    27.4\% &                                  1.60 \\
       \covidFact &         COVID-19 &              Reddit posts &                    Automatic &                       903 &                      313 &                    12.4\% &                                  1.70 \\
       \healthVer &         COVID-19 &       Retrieved documents &          Naturally occurring &                     1,622 &                      230 &                    14.9\% &                                  1.40 \\
\bottomrule
\end{tabular}


==> table/fewshot_results.tex <==
\begin{tabular}{
    p{0.075\linewidth}
    p{0.1\linewidth}
    p{0.03\linewidth}
    P{0.026\linewidth}P{0.026\linewidth}P{0.033\linewidth}  P{0.026\linewidth}P{0.026\linewidth}P{0.033\linewidth} P{0.001\linewidth}
    P{0.026\linewidth}P{0.026\linewidth}P{0.033\linewidth}  P{0.026\linewidth}P{0.026\linewidth}P{0.033\linewidth} P{0.001\linewidth}
    P{0.026\linewidth}P{0.026\linewidth}P{0.033\linewidth}  P{0.026\linewidth}P{0.026\linewidth}P{0.033\linewidth} P{0.001\linewidth}
    }
    \toprule

                               &                             & {}    & \multicolumn{6}{c}{\textbf{\healthVer}} &                              & \multicolumn{6}{c}{\textbf{\covidFact}} &                              & \multicolumn{6}{c}{\textbf{\scifact}} &                                                                                                                                                                                                                                    \\
                               &                             & {}    & \multicolumn{3}{c}{Abstract}            & \multicolumn{3}{c}{Sentence} &                                         & \multicolumn{3}{c}{Abstract} & \multicolumn{3}{c}{Sentence}          &               & \multicolumn{3}{c}{Abstract} & \multicolumn{3}{c}{Sentence}                                                                                                                                                        \\
    \cmidrule(lr){4-6} \cmidrule(lr){7-9} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){18-20} \cmidrule(lr){21-23}
    Setting                    & Model                       & Sci & \sz{P}                                  & \sz{R}                       & F1                                      & \sz{P}                       & \sz{R}                                & F1            &                              & \sz{P}                       & \sz{R}    & F1            & \sz{P}    & \sz{R}    & F1            &  & \sz{P}    & \sz{R}    & F1            & \sz{P}    & \sz{R}    & F1            \\
    \midrule
    \multirow{4}{*}{Zero-shot} & \tworows{\textsc{Paragraph}                                                                                                                                                                                                                                                                                                                                                                                                                                        \\ \textsc{Joint}}  & \xmark  & \sz{66.7}                               & \sz{3.0}                     & 5.8                                     & \sz{33.3}                    & \sz{0.9}                              & 1.8  &                              & \sz{73.9}                    & \sz{5.4}  & 10.0 & \sz{39.1} & \sz{1.7}  & 3.2  &  & \sz{59.5} & \sz{11.3} & 18.9 & \sz{48.9} & \sz{6.2}  & 11.0 \\
                               &                             & \cmark   & \sz{72.3}                               & \sz{14.4}                    & 24.0                                    & \sz{22.9}                    & \sz{2.7}                              & 4.9           &                              & \sz{51.3}                    & \sz{37.9} & 43.6          & \sz{31.5} & \sz{16.0} & 21.3          &  & \sz{52.9} & \sz{32.4} & 40.2          & \sz{36.4} & \sz{14.9} & 21.1          \\
    \cmidrule(lr){2-23}
                               & \tworows{\textsc{Long}                                                                                                                                                                                                                                                                                                                                                                                                                                             \\ \textsc{Checker}} & \xmark  & \sz{80.0}                               & \sz{0.7}                     & 1.3                                     & \sz{66.7}                    & \sz{0.4}                              & 0.7  &                              & \sz{95.8}                    & \sz{14.5} & 25.2 & \sz{63.5} & \sz{6.2}  & 11.2 &  & \sz{83.8} & \sz{14.0} & 23.9 & \sz{64.9} & \sz{6.5}  & 11.8 \\
                               &                             & \cmark   & \sz{60.6}                               & \sz{20.5}                    & \textbf{30.7}                           & \sz{25.0}                    & \sz{4.6}                              & \textbf{7.8}  &                              & \sz{48.8}                    & \sz{45.7} & \textbf{47.2} & \sz{32.7} & \sz{18.5} & \textbf{23.6} &  & \sz{49.0} & \sz{44.6} & \textbf{46.7} & \sz{39.0} & \sz{21.6} & \textbf{27.8} \\
    \cmidrule(lr){1-23}
    \multirow{4}{*}{Few-shot}  & \tworows{\textsc{Paragraph}                                                                                                                                                                                                                                                                                                                                                                                                                                        \\ \textsc{Joint}}  & \xmark  & \sz{57.2}                               & \sz{38.2}                    & 45.9                                    & \sz{35.0}                    & \sz{23.3}                             & 28.0 &                              & \sz{65.7}                    & \sz{29.6} & 40.9 & \sz{41.1} & \sz{13.8} & 20.7 &  & \sz{50.0} & \sz{39.6} & 44.2 & \sz{32.1} & \sz{23.2} & 27.0 \\
                               &                             & \cmark   & \sz{62.7}                               & \sz{41.6}                    & 50.0                                    & \sz{46.0}                    & \sz{29.3}                             & 35.8          &                              & \sz{73.3}                    & \sz{60.6} & 66.3          & \sz{44.3} & \sz{30.6} & 36.2          &  & \sz{44.4} & \sz{51.4} & 47.6          & \sz{33.0} & \sz{35.1} & 34.0          \\
    \cmidrule(lr){2-23}
                               & \tworows{\textsc{Long}                                                                                                                                                                                                                                                                                                                                                                                                                                             \\ \textsc{Checker}} & \xmark  & \sz{56.4}                               & \sz{50.8}                    & 53.4                                    & \sz{35.6}                    & \sz{28.4}                             & 31.6 &                              & \sz{74.5}                    & \sz{74.5} & \textbf{74.5} & \sz{39.5} & \sz{45.1} & \textbf{42.1} &  & \sz{72.4} & \sz{43.7} & 54.5 & \sz{48.8} & \sz{32.4} & 39.0 \\
                               &                             & \cmark   & \sz{63.6}                               & \sz{47.9}                    & \textbf{54.7}                           & \sz{44.0}                    & \sz{30.7}                             & \textbf{36.1} &                              & \sz{71.3}                    & \sz{68.1} & 69.7 & \sz{40.5} & \sz{35.1} & 37.6 &  & \sz{76.4} & \sz{54.0} & \textbf{63.3} & \sz{51.7} & \sz{40.3} & \textbf{45.3} \\
    \bottomrule
\end{tabular}


==> table/fewshot_results_orig.tex <==
\begin{tabular}{lllllllllllllllllllll}
\toprule
         &             & {} & abstract_label_only_precision & abstract_label_only_recall & abstract_label_only_f1 & sentence_label_precision & sentence_label_recall & sentence_label_f1 & abstract_label_only_precision & abstract_label_only_recall & abstract_label_only_f1 & sentence_label_precision & sentence_label_recall & sentence_label_f1 & abstract_label_only_precision & abstract_label_only_recall & abstract_label_only_f1 & sentence_label_precision & sentence_label_recall & sentence_label_f1 \\
         &             & dataset &                     healthver &                  healthver &              healthver &                healthver &             healthver &         healthver &                    covid_fact &                 covid_fact &             covid_fact &               covid_fact &            covid_fact &        covid_fact &                       scifact &                    scifact &                scifact &                  scifact &               scifact &           scifact \\
setting & model & adapt &                               &                            &                        &                          &                       &                   &                               &                            &                        &                          &                       &                   &                               &                            &                        &                          &                       &                   \\
\midrule
\multirow{4}{*}{Zero-shot} & \multirow{2}{*}{\pjoint} & fever &                     \sz{66.7} &                   \sz{3.0} &                    5.8 &                \sz{33.3} &              \sz{0.9} &               1.8 &                     \sz{73.9} &                   \sz{5.4} &                   10.0 &                \sz{39.1} &              \sz{1.7} &               3.2 &                     \sz{59.5} &                  \sz{11.3} &                   18.9 &                \sz{48.9} &              \sz{6.2} &              11.0 \\
         &             & all &                     \sz{72.3} &                  \sz{14.4} &                   24.0 &                \sz{22.9} &              \sz{2.7} &               4.9 &                     \sz{51.3} &                  \sz{37.9} &                   43.6 &                \sz{31.5} &             \sz{16.0} &              21.3 &                     \sz{52.9} &                  \sz{32.4} &                   40.2 &                \sz{36.4} &             \sz{14.9} &              21.1 \\
\cline{2-21}
         & \multirow{2}{*}{\sysname} & fever &                     \sz{80.0} &                   \sz{0.7} &                    1.3 &                \sz{66.7} &              \sz{0.4} &               0.7 &                     \sz{95.8} &                  \sz{14.5} &                   25.2 &                \sz{63.5} &              \sz{6.2} &              11.2 &                     \sz{83.8} &                  \sz{14.0} &                   23.9 &                \sz{64.9} &              \sz{6.5} &              11.8 \\
         &             & all &                     \sz{60.6} &                  \sz{20.5} &                   30.7 &                \sz{25.0} &              \sz{4.6} &               7.8 &                     \sz{48.8} &                  \sz{45.7} &                   47.2 &                \sz{32.7} &             \sz{18.5} &              23.6 &                     \sz{49.0} &                  \sz{44.6} &                   46.7 &                \sz{39.0} &             \sz{21.6} &              27.8 \\
\cline{1-21}
\cline{2-21}
\multirow{4}{*}{Few-shot} & \multirow{2}{*}{\pjoint} & fever &                     \sz{57.2} &                  \sz{38.2} &                   45.9 &                \sz{35.0} &             \sz{23.3} &              28.0 &                     \sz{65.7} &                  \sz{29.6} &                   40.9 &                \sz{41.1} &             \sz{13.8} &              20.7 &                     \sz{50.0} &                  \sz{39.6} &                   44.2 &                \sz{32.1} &             \sz{23.2} &              27.0 \\
         &             & all &                     \sz{62.7} &                  \sz{41.6} &                   50.0 &                \sz{46.0} &             \sz{29.3} &              35.8 &                     \sz{73.3} &                  \sz{60.6} &                   66.3 &                \sz{44.3} &             \sz{30.6} &              36.2 &                     \sz{44.4} &                  \sz{51.4} &                   47.6 &                \sz{33.0} &             \sz{35.1} &              34.0 \\
\cline{2-21}
         & \multirow{2}{*}{\sysname} & fever &                     \sz{56.4} &                  \sz{50.8} &                   53.4 &                \sz{35.6} &             \sz{28.4} &              31.6 &                     \sz{74.5} &                  \sz{74.5} &                   74.5 &                \sz{39.5} &             \sz{45.1} &              42.1 &                     \sz{72.4} &                  \sz{43.7} &                   54.5 &                \sz{48.8} &             \sz{32.4} &              39.0 \\
         &             & all &                     \sz{63.6} &                  \sz{47.9} &                   54.7 &                \sz{44.0} &             \sz{30.7} &              36.1 &                     \sz{71.3} &                  \sz{68.1} &                   69.7 &                \sz{40.5} &             \sz{35.1} &              37.6 &                     \sz{76.4} &                  \sz{54.0} &                   63.3 &                \sz{51.7} &             \sz{40.3} &              45.3 \\
\bottomrule
\end{tabular}


==> table/fewshot_results_wrapper.tex <==
\begin{table*}[t]
  \footnotesize
  \setlength{\tabcolsep}{0.3em}
  \centering

  \input{table/fewshot_results.tex}

  \caption{Performance of \sysname and \pjoint in the zero-shot and few-shot settings. Rows where ``Sci'' is marked \cmark indicate that the model was pretrained on scientific data. Rows marked \xmark indicate pretraining on \fever only. The results show that in-domain pretraining improves performance, and that \sysname outperforms \pjoint.}

  \label{tbl:fewshot_results}

\end{table*}


==> table/human_performance_orig.tex <==
\begin{tabular}{lrrlrrl}
\toprule
{} & \multicolumn{3}{l}{Abstract} & \multicolumn{3}{l}{Sentence} \\
{} &        P &     R &             F1 &        P &     R &             F1 \\
\midrule
\vertserini &     90.7 &  74.3 &  \textbf{81.7} &     79.6 &  62.2 &           69.8 \\
\pjoint     &     87.2 &  64.4 &           74.1 &     76.7 &  55.1 &           64.1 \\
\sysname    &     87.4 &  75.2 &           80.9 &     80.5 &  70.3 &  \textbf{75.0} \\
Human       &     94.8 &  84.1 &           89.1 &     67.4 &  67.4 &           67.4 \\
\bottomrule
\end{tabular}


==> table/negative_sampling_orig.tex <==
\begin{tabular}{llrrrrrr}
\toprule
     &        & \multicolumn{3}{c}{Abstract-Level} & \multicolumn{3}{c}{Sentence-Level} \\
     &        & \multicolumn{3}{c}{Label-Only} & \multicolumn{3}{c}{Selection+Label} \\
     &        &              P &    R &   F1 &               P &    R &   F1 \\
Retrieval & Neg. sampling &                &      &      &                 &      &      \\
\midrule
\multirow{2}{*}{Oracle} & \xmark &           81.9 & 85.6 & 83.7 &            69.5 & 69.7 & 69.6 \\
     & \cmark &           85.2 & 75.2 & 79.9 &            79.0 & 70.3 & 74.4 \\
\cline{1-8}
\multirow{2}{*}{Open} & \xmark &           38.9 & 80.6 & 52.5 &            35.4 & 65.1 & 45.9 \\
     & \cmark &           73.8 & 71.2 & 72.5 &            67.4 & 67.0 & 67.2 \\
\bottomrule
\end{tabular}



==> table/scifact_context_test_f1.tex <==
\begin{tabular}{
    p{0.30\linewidth}
    R{0.080\linewidth}R{0.080\linewidth}P{0.0005\linewidth}
    R{0.080\linewidth}R{0.080\linewidth}P{0.0005\linewidth}
    R{0.080\linewidth}R{0.080\linewidth}
    }
    \toprule
    {}          & \multicolumn{2}{c}{\tworows{Stand- \\ alone}} &               & \multicolumn{2}{c}{\tworows{Context- \\dependent}} &               & \multicolumn{2}{c}{\tworows{All}}                                    \\
    & & & & & & & & \\
    \cmidrule(lr){2-3}     \cmidrule(lr){5-6}     \cmidrule(lr){8-9}
    {}          & Abst                           & Sent          &                             & Abst          & Sent                    &  & Abst          & Sent          \\
    \midrule
    \vertserini & \textbf{87.8}                  & 75.6          &                             & 75.2          & 67.0                    &  & \textbf{79.7} & 70.0          \\
    \pjoint     & 85.0                           & \textbf{77.4} &                             & 73.1          & 64.0                    &  & 77.3          & 68.8          \\
    \arrayrulecolor{black!30}\cmidrule(lr){1-9} \arrayrulecolor{black!100}
    \sysname    & 80.5                           & 69.6          &                             & \textbf{78.4} & \textbf{71.0}           &  & 79.2          & \textbf{70.5} \\
    \midrule
    Count       & \multicolumn{2}{l}{43}         &               & \multicolumn{2}{l}{85}      &               & \multicolumn{2}{l}{128}                                    \\
    \bottomrule
\end{tabular}


==> table/scifact_context_test_f1_orig.tex <==
\begin{tabular}{lrrrrrr}
\toprule
{} & \multicolumn{2}{c}{No-context} & \multicolumn{2}{c}{Context} & \multicolumn{2}{c}{All} \\
{} &   Abstract & Sentence & Abstract & Sentence & Abstract & Sentence \\
{} &         F1 &       F1 &       F1 &       F1 &       F1 &       F1 \\
\midrule
vert5erini      &       87.8 &     75.6 &     75.2 &     67.0 &     79.7 &     70.0 \\
paragraph_joint &       85.0 &     77.4 &     73.1 &     64.0 &     77.3 &     68.8 \\
longformer_20   &       80.5 &     69.6 &     78.4 &     71.0 &     79.2 &     70.5 \\
\bottomrule
\end{tabular}



==> table/scifact_context_test_f1_wrapper.tex <==
\begin{table}[t]
  \footnotesize
  \setlength{\tabcolsep}{0.3em}
  \centering

\input{table/scifact_context_test_f1.tex}

\caption{
  Performance of models on \scifact instances with rationales that are ``Stand-alone'' (can be interpreted correctly out-of-context) and ``Context-dependent'' (require abstract context to be interpreted correctly). The ``All'' column shows performance on all instances combined. ``Abst'' and ``Sent'' indicate abstract-level and sentence-level F1. \sysname exhibits the strongest performance on context-dependent rationales.
}
    \label{tbl:scifact_context}

\end{table}


==> table/skills_acronym_raw.tex <==
\begin{tabular}{lrrrrrr}
\toprule
{} &  abstract\_label\_only\_precision &  abstract\_label\_only\_recall &  abstract\_label\_only\_f1 &  abstract\_label\_only\_precision &  abstract\_label\_only\_recall &  abstract\_label\_only\_f1 \\
model               &                                &                             &                         &                                &                             &                         \\
\midrule
longchecker         &                           88.1 &                        73.8 &                    80.3 &                           86.0 &                        77.1 &                    81.3 \\
longformer\_pipe\_v2  &                           89.9 &                        77.5 &                    83.2 &                           88.6 &                        81.2 &                    84.8 \\
longchecker\_as\_pipe &                           97.1 &                        42.5 &                    59.1 &                           85.0 &                        35.4 &                    50.0 \\
\bottomrule
\end{tabular}


==> table/skills_context_raw.tex <==
\begin{tabular}{lrrrrrr}
\toprule
{} &  abstract_label_only_precision &  abstract_label_only_recall &  abstract_label_only_f1 &  abstract_label_only_precision &  abstract_label_only_recall &  abstract_label_only_f1 \\
model               &                                &                             &                         &                                &                             &                         \\
\midrule
longchecker         &                           86.1 &                        82.9 &                    84.5 &                           90.3 &                        60.9 &                    72.7 \\
longformer_pipe_v2  &                           92.4 &                        89.0 &                    90.7 &                           82.4 &                        60.9 &                    70.0 \\
longchecker_as_pipe &                           91.8 &                        54.9 &                    68.7 &                          100.0 &                        13.0 &                    23.1 \\
\bottomrule
\end{tabular}

